Schrodinger dynamics and Berry phase of undulatory locomotion

Spectral mode representations play an essential role in various areas of physics, from quantum mechanics to fluid turbulence, but they are not yet extensively used to characterize and describe the behavioral dynamics of living systems. Here, we show that mode-based linear models inferred from experimental live-imaging data can provide an accurate low-dimensional description of undulatory locomotion in worms, centipedes, robots, and snakes. By incorporating physical symmetries and known biological constraints into the dynamical model, we find that the shape dynamics are generically governed by Schrodinger equations in mode space. The eigenstates of the effective biophysical Hamiltonians and their adiabatic variations enable the efficient classification and differentiation of locomotion behaviors in natural, simulated, and robotic organisms using Grassmann distances and Berry phases. While our analysis focuses on a widely studied class of biophysical locomotion phenomena, the underlying approach generalizes to other physical or living systems that permit a mode representation subject to geometric shape constraints.

==> SIextras.tex <==
% \section{Distance between vector spaces}

% The dominant two eigenvectors $\mathbf{v}_1$ and $\mathbf{w}_1$ define a two-dimensional subspace of $n$-dimensional vectors $\mathbf{u}_k = \alpha_1 \mathbf{v}_1 + \beta_1 \mathbf{w}_1$. We define the distance between two subspaces by the minimum norm vector that exists in their combined span, a measure of how linearly dependent the two spaces are, 
% \begin{align*}
%     D(\mathbf{v}_1, \mathbf{w}_1, \mathbf{v}_2, \mathbf{w}_2) &= \min_{\alpha_1, \beta_1, \alpha_2, \beta_2}  \left\lVert \begin{bmatrix}
%     \vdots & \vdots & \vdots & \vdots \\
%     \mathbf{v}_1 &  \mathbf{w}_1 & 
%     \mathbf{v}_2 & \mathbf{w}_2  \\
%     \vdots & \vdots & \vdots & \vdots
%     \end{bmatrix}
%     \begin{bmatrix}
%     \alpha_1 \\ \beta_1 \\ \alpha_2 \\ \beta_2
%     \end{bmatrix}
%     \right\rVert_2^2 \\
%     &= \min_{\alpha_1, \beta_1, \alpha_2, \beta_2} \begin{bmatrix}
%     \alpha_1 & \beta_1 & \alpha_2 & \beta_2
%     \end{bmatrix}
%     \begin{bmatrix}
%     \cdots & \mathbf{v}_1^\dagger & \cdots \\  \cdots & \mathbf{w}_1^\dagger & \cdots \\
%     \cdots & \mathbf{v}_2^\dagger & \cdots \\ \cdots & \mathbf{w}_2^\dagger & \cdots 
%     \end{bmatrix}
%     \begin{bmatrix}
%     \vdots & \vdots & \vdots & \vdots \\
%     \mathbf{v}_1 &  \mathbf{w}_1 & 
%     \mathbf{v}_2 & \mathbf{w}_2  \\
%     \vdots & \vdots & \vdots & \vdots
%     \end{bmatrix}
%     \begin{bmatrix}
%     \alpha_1 \\ \beta_1 \\ \alpha_2 \\ \beta_2
%     \end{bmatrix} \\ 
%     &= \min_{\alpha_1, \beta_1, \alpha_2, \beta_2} \begin{bmatrix}
%     \alpha_1 & \beta_1 & \alpha_2 & \beta_2
%     \end{bmatrix}
%     \begin{bmatrix}
%     \mathbf{v}_1^\dagger \mathbf{v}_1 & \mathbf{v}_1^\dagger \mathbf{w}_1 & \mathbf{v}_1^\dagger \mathbf{v}_2 & \mathbf{v}_1^\dagger \mathbf{w}_2 \\
%      \mathbf{w}_1^\dagger \mathbf{v}_1 & \mathbf{w}_1^\dagger \mathbf{w}_1 & \mathbf{w}_1^\dagger \mathbf{v}_2 & \mathbf{w}_1^\dagger \mathbf{w}_2 \\
%       \mathbf{v}_2^\dagger \mathbf{v}_1 & \mathbf{v}_2^\dagger \mathbf{w}_1 & \mathbf{v}_2^\dagger \mathbf{v}_2 & \mathbf{v}_2^\dagger \mathbf{w}_2 \\
%       \mathbf{w}_2^\dagger \mathbf{v}_1 & \mathbf{w}_2^\dagger \mathbf{w}_1 & \mathbf{w}_2^\dagger \mathbf{v}_2 & \mathbf{w}_2^\dagger \mathbf{w}_2
%     \end{bmatrix}
%     \begin{bmatrix}
%     \alpha_1 \\ \beta_1 \\ \alpha_2 \\ \beta_2
%     \end{bmatrix} \\
%     &= \min_{\mathbf{c}} \mathbf{c}^\dagger V \mathbf{c}
% \end{align*}
% since the inner-product in the final matrix is symmetric, for example $\mathbf{v}_1^\dagger \mathbf{w}_2 = \mathbf{w}_2^\dagger \mathbf{v}_1$ and $D(\mathbf{v}_1, \mathbf{w}_1, \mathbf{v}_2, \mathbf{w}_2) \ge 0$ the matrix $V$ is symmetric positive semi-definite. To avoid the trivial minimum when $\mathbf{c} = \boldsymbol{0}$ we further constrain $\mathbf{c}^\dagger \mathbf{c} = 1$. The well known result of minimizing quadratic forms over a sphere then given the minimum as the smallest magnitude eigenvector of $V$, 
% \begin{equation}
%      D(\mathbf{v}_1, \mathbf{w}_1, \mathbf{v}_2, \mathbf{w}_2) = \text{eigmin} V
% \end{equation}
% Although we consider distances between two dimensional spans here the formulation can be generalized readily to more vectors. 

% \begin{align}
%     \mathbf{r}(s,t) = 
%     \begin{bmatrix}
%     x(s,t)\\
%     y(s,t)
%     \end{bmatrix} = \sum_{n=0}^N
%     \begin{bmatrix}
%     \hat{x}_n(t)\\
%     \hat{y}_n(t)
%     \end{bmatrix}T_n(s) = \begin{bmatrix}
%     \hat{x}_0(t)\\
%     \hat{y}_0(t)
%     \end{bmatrix} + \sum_{n=1}^N
%     \begin{bmatrix}
%     (\hat{\boldsymbol{\psi}}_x)_n(t)\\
%     (\hat{\boldsymbol{\psi}}_y)_n(t)
%     \end{bmatrix}T_n(s)
% \end{align}
% where we use the fact that $T_0(s) = 1$. Defining the Chebyshev vector $\mathbf{T}(s) = [T_1(s),\, T_2(s),\, \cdots,\,T_N(s)]$, we can write 
% \begin{equation}
%     \mathbf{r}(s,t) - \boldsymbol{\psi}_0(t) = \ell \left\{ \begin{bmatrix}
%     c_{0,1} \\
%     d_{0,1} \end{bmatrix} (L^{-1})^\dagger \mathbf{v}_0(t) + \sum_{k=1}^K
%     \begin{bmatrix}
%     c_{k,1} \\ d_{k, 1} \end{bmatrix} \left(L^{-1}\right)^\dagger\tilde{\mathbf{v}}_k(t)  + \begin{bmatrix} c_{k,2} \\
%     d_{k,2} \end{bmatrix} \left(L^{-1}\right)^\dagger\tilde{\mathbf{w}}_k(t) \right\} \cdot \mathbf{T}(s).
% \end{equation}
% Now, defining $\hat{\mathbf{v}}_k = \ell (L^{-1})^\dagger \mathbf{v}_k$ and $\hat{\mathbf{w}}_k = \ell (L^{-1})^\dagger \mathbf{w}_k$ and plugging in our definition for $\tilde{\mathbf{v}}$ and $\tilde{\mathbf{w}}$ gives
% \begin{equation}
%     \mathbf{r}(s,t) - \boldsymbol{\psi}_0(t) = \sum_{n=1}^N  \left\{\begin{bmatrix} c_{0, 1} \\ d_{0, 1} \end{bmatrix} + \sum_{k=1}^K 
%     \begin{bmatrix}
%     c_{k,1} \\ d_{k, 1} \end{bmatrix} (\cos{(\lambda_kt)}\hat{v}_{n,k}-\sin{(\lambda_kt)}\hat{w}_{n,k}) + \begin{bmatrix} c_{k,2} \\
%      d_{k,2}
%     \end{bmatrix} (\cos{(\lambda_kt)}\hat{w}_{n,k}+\sin{(\lambda_kt)}\hat{v}_{n,k}) \right\}T_n(s).
% \end{equation}
% idealized locomotion state

% Consider now the state where we enforce that the $\lambda_k = k \lambda$ are interger multiples of some base frequency, 
% \begin{equation}
%      x(s, t) - x_0(t) =\sum_{n=1}^N \left[ c_{0}v_{n, 0} +  \sum_{k=1}^K
%     \left[c_{k,1}(\cos{(k \lambda t)}v_{n,k}-\sin{(k \lambda t)}w_{n,k}) + c_{k,2}(\cos{(k \lambda t)}w_{n,k}+\sin{(k \lambda t)}v_{n,k}) \right] \right] T_n(s).
% \end{equation}
% We can calculate the time average square of $x(s, t)$ over a single period
% \begin{align*}
%     \langle (x - x_0)^2 \rangle_t (s) &=  \frac{\lambda}{2\pi} \int_{0}^{\frac{2\pi}{\lambda}} \mathrm{d}t\, x(s, t)^2 \\ 
%     %
%     &= \frac{\lambda}{2\pi} \int_{0}^{\frac{2\pi}{\lambda}} \mathrm{d}t\,
%     \sum_{k=0}^K \sum_{n=0}^N \sum_{l=0}^K \sum_{m=0}^N
%     \left[c_{k,1}(\cos{(k \lambda t)}v_{n,k}-\sin{(k \lambda t)}w_{n,k}) + c_{k,2}(\cos{(k \lambda t)}w_{n,k}+\sin{(k \lambda t)}v_{n,k}) \right] \\ &\hspace{8em} \left[c_{l,1}(\cos{(l \lambda t)}v_{m,l}-\sin{(l \lambda t)}w_{m, l}) + c_{l,2}(\cos{(l \lambda t)}w_{m,l}+\sin{(l \lambda t)}v_{m,l}) \right] T_n(s) T_m(s) \\ 
%     %
%     &= \frac{\lambda}{2\pi} \int_{0}^{\frac{2\pi}{\lambda}} \mathrm{d}t\,
%     \sum_{k=0}^K \sum_{n=0}^N \sum_{l=0}^K \sum_{m=0}^N \\ &\hspace{6em}
%     \left[ c_{k, 1} c_{l, 1} v_{n, k} v_{m, l} + c_{k, 2} c_{l, 2} w_{n, k} w_{m, l} + c_{k, 2} c_{l, 1} w_{n, k} v_{m, l} + c_{k, 1} c_{l, 2} v_{n, k} w_{m, l}  \right] \cos(k \lambda t) \cos(l \lambda t) \\ &\hspace{5em} + 
%     \left[ c_{k, 1} c_{l, 1} w_{n, k} w_{m, l} + c_{k, 2} c_{l, 2} v_{n, k} v_{m, l} - c_{k, 2} c_{l, 1} v_{n, k} w_{m, l} - c_{k, 1} c_{l, 2} w_{n, k} v_{m, l} \right] \sin(k \lambda t) \sin(l \lambda t) \\ &\hspace{5em}+ 
%     \left[ \cdot \right] \sin(k \lambda t) \cos(l \lambda t) + 
%     \left[ \cdot \right] \cos(k \lambda t) \sin(l \lambda t) \\
%     \intertext{now utilizing the orthogonality of $\sin$ and $\cos$ we find the last two terms vanish and we have, }
%     &= \frac{1}{2} \sum_{k=0}^K \sum_{n=0}^N \sum_{l=0}^K \sum_{m=0}^N
%     \left[ c_{k, 1} c_{l, 1} v_{n, k} v_{m, l} + c_{k, 2} c_{l, 2} w_{n, k} w_{m, l} + c_{k, 2} c_{l, 1} w_{n, k} v_{m, l} + c_{k, 1} c_{l, 2} v_{n, k} w_{m, l}  \right] (\delta_{l, k} + \delta_{l, 0}\delta_{k, 0})  \\ &\hspace{5em} +
%     \left[ c_{k, 1} c_{l, 1} w_{n, k} w_{m, l} + c_{k, 2} c_{l, 2} v_{n, k} v_{m, l} - c_{k, 2} c_{l, 1} v_{n, k} w_{m, l} - c_{k, 1} c_{l, 2} w_{n, k} v_{m, l} \right] (\delta_{l, k} - \delta_{l, 0}\delta_{k, 0}) \\
%     &= \frac{1}{2} \sum_{k=0}^K \sum_{n=0}^N \sum_{m=0}^N \left[ c_{k, 1}^2 v_{n, k} v_{m, k} + c_{k, 2}^2 w_{n, k} w_{m, k} + c_{k, 2} c_{k, 1} \left(w_{n, k} v_{m, k} + v_{n, k} w_{m, k}\right)  \right](1 + \delta_{k, 0}) \\ &\hspace{5em} +
%     \left[ c_{k, 1}^2 w_{n, k} w_{m, k} + c_{k, 2}^2 v_{n, k} v_{m, k} - c_{k, 2} c_{k, 1} \left(v_{n, k} w_{m, k} +  w_{n, k} v_{m, k}\right) \right] (1 - \delta_{k, 0}) \\
%     &=\sum_{n=1}^N \sum_{m=1}^N \left[ c_{0, 1}^2 v_{n, 0}v_{m, 0} + \frac{1}{2} \sum_{k=1}^K (c_{k, 1}^2 + c_{k, 2}^2) (v_{n, k} v_{m, k} + w_{n, k} w_{m, k}) \right]T_n(s) T_m(s) \\
%     &= v_0(s)^2 + \frac{1}{2} \sum_{k} (c_{k, 1}^2 + c_{k, 2}^2) \left[v_k(s)^2 + w_k(s)^2\right]
% \end{align*}

\usepackage{verbatim}

\newcommand{\detailtexcount}[1]{%
  \immediate\write18{texcount -merge -sum=1,1,1,0,238.5,1,32 -q #1.tex > #1.wcdetail }%
  \verbatiminput{#1.wcdetail}}
  \detailtexcount{main}

%TC:macro \caption [option:text,text]


%% Information 
\rv{To fit the data to these dynamics we seek to minimize the objective function,
\begin{align*} \label{SIeq:full_dynamics_loss}
L(\{Z_k\}, \{\lambda_k\}) &= \frac{1}{T}\sum_{m = 1}^T \left\lVert \sum_{k = 1}^{n'} Z_k \exp(t_m \Lambda_k) (Z_k^\top \boldsymbol{\psi}_0) - \boldsymbol{\psi}(t_m) \right\rVert_F^2 \\
&= \frac{1}{T}\sum_{m = 1}^T \sum_{k = 1}^{n'}  \Bigg[\sum_{l = 1}^{n'} \boldsymbol{\psi}_0^\top Z_k \exp(-t_m \Lambda_k) Z_k^\top Z_l\exp(t_m \Lambda_l) Z_l^\top \boldsymbol{\psi}_0 -  \boldsymbol{\psi}(t_m)^\top Z_k \exp(t_m \Lambda_k) Z_k^\top \boldsymbol{\psi}_0 \\
&\qquad \qquad \qquad\qquad- \boldsymbol{\psi}_0^\top Z_k \exp(-t_m \Lambda_k) Z_k^\top \boldsymbol{\psi}(t_m) + \frac{1}{n}\boldsymbol{\psi}(t_m)^\top \boldsymbol{\psi}(t_m) \Bigg] \\ 
&= \left\langle\left\lvert \boldsymbol{\psi}(t_m) \right\rvert^2\right\rangle_1 + \sum_{k = 1}^{n'}\boldsymbol{\psi}_0^\top Z_k Z_k^\top \boldsymbol{\psi}_0 - 2\sum_{m = 1}^T \sum_{k = 1}^{n'}\boldsymbol{\psi}(t_m)^\top Z_k \exp(t_m \Lambda_k) Z_k^\top \boldsymbol{\psi}_0.
\end{align*}
We use the notation $\langle f(t) \rangle_{g(t)}$ to represent the discrete time average $\frac{1}{T}\sum_{m = 1}^{T} g(t_m) f(t_m)$ with respect to the weight function $g(t)$. 
}
\rv{We can rewrite the loss as a quadratic form in terms of the unknowns $\mathbf{z}_k$, the second term becomes,
\begin{align*}
\boldsymbol{\psi}_0^\top Z_k Z_k^\top \boldsymbol{\psi}_0 = \begin{bmatrix} \boldsymbol{\psi}_0^\top \mathbf{z}_k & \boldsymbol{\psi}_0^\top \mathbb{P}_n \mathbf{z}_k \end{bmatrix} \begin{bmatrix} \mathbf{z}_k^\top \boldsymbol{\psi}_0 \\  -\mathbf{z}_k^\top \mathbb{P}_n \boldsymbol{\psi}_0 \end{bmatrix} = \mathbf{z}_k^\top \left[\boldsymbol{\psi}_0 \boldsymbol{\psi}_0^\top - \mathbb{P}_n \boldsymbol{\psi}_0 \boldsymbol{\psi}_0^\top \mathbb{P}_n\right] \mathbf{z}_k
\end{align*}
and the third term becomes,
\begin{align*}
\boldsymbol{\psi}(t_m)^\top Z_k \exp(t_m \Lambda_k) Z_k^\top \boldsymbol{\psi}_0 &= \begin{bmatrix} \boldsymbol{\psi}_m^\top \mathbf{z}_k & -\left(\mathbb{P}_n \boldsymbol{\psi}_m\right)^\top \mathbf{z}_k \end{bmatrix} \begin{bmatrix} \cos \lambda_k t_m  & \sin \lambda_k t_m \\ -\sin \lambda_k t_m & \cos \lambda_k t_m\end{bmatrix} \begin{bmatrix} \mathbf{z}_k^\top \boldsymbol{\psi}_0 \\  -\mathbf{z}_k^\top \mathbb{P}_n \boldsymbol{\psi}_0 \end{bmatrix} \\
&= \mathbf{z}_k^\top \big\{\boldsymbol{\psi}_0 \left[\cos(\lambda_k t_m) \boldsymbol{\psi}(t_m) + \sin(\lambda_k t_m)  \mathbb{P}_n\boldsymbol{\psi}(t_m) \right]^\top - \\
&\qquad\qquad\mathbb{P}_n \boldsymbol{\psi}_0 \left[\sin(\lambda_k t_m) \boldsymbol{\psi}(t_m) - \cos(\lambda_k t_m)  \mathbb{P}_n\boldsymbol{\psi}(t_m) \right]^\top \big\} \mathbf{z}_k \\
&= \mathbf{z}_k^\top \big\{\boldsymbol{\psi}_0 \left[\cos(\lambda_k t_m) \boldsymbol{\psi}(t_m) + \sin(\lambda_k t_m)  \mathbb{P}_n\boldsymbol{\psi}(t_m) \right]^\top - \\
&\qquad\qquad\mathbb{P}_n \boldsymbol{\psi}_0 \left[\cos(\lambda_k t_m) \boldsymbol{\psi}(t_m) + \sin(\lambda_k t_m) \mathbb{P}_n\boldsymbol{\psi}(t_m)\right]^\top \mathbb{P}_n \big\} \mathbf{z}_k .
\end{align*}
The symmetric quadratic form of the loss depends on the rank-$1$ matrix 
\begin{equation}
D_k =  \boldsymbol{\psi}_0\left[-\frac{1}{2} \boldsymbol{\psi}_0 + \left\langle \boldsymbol{\psi} \right\rangle_{\cos \lambda_k t} + \mathbb{P}_n \left\langle \boldsymbol{\psi} \right\rangle_{\sin \lambda_k t} \right]^\top
\end{equation}
and its permutations, through 
\begin{align*}
L(\{\mathbf{z}_k\}, \{\lambda_k\}) &= \left\langle |\boldsymbol{\psi}|^2 \right\rangle_1  -\sum_{k = 1}^n \mathbf{z}_k^\top \left[D_k + D_k^\top + \mathbb{P}_n \left(D_k + D_k^\top\right) \mathbb{P}_n^\top \right] \mathbf{z}_k \\
&= \left\langle |\boldsymbol{\psi}|^2 \right\rangle_1  -\sum_{k = 1}^n \mathbf{z}_k^\top L_k \mathbf{z}_k
%\left|\boldsymbol{\psi}_0\right|^2
\end{align*}
subject to constraints on $\mathbf{z}_k$ so that $Z_K$ satisfies $Z_l^\top Z_k = \delta_{k, l} \mathbb{I}_2$. The loss is quadratic in $\mathbf{z}_k$ allowing us to calculate the minimum using the eigendecomposition of the matrix for fixed $\lambda_k$. 
% \begin{align}
% \boldsymbol{\psi}_0^\top Z_k Z_k^\top \boldsymbol{\psi}_0 &= \begin{bmatrix} (\boldsymbol{\psi}^x_0)^\top \mathbf{x}_k + (\boldsymbol{\psi}^y_0)^\top \mathbf{y}_k &  (\boldsymbol{\psi}^x_0)^\top \mathbf{y}_k  -(\boldsymbol{\psi}^y_0)^\top \mathbf{x}_k\end{bmatrix} \begin{bmatrix} \mathbf{x}_k^\top (\boldsymbol{\psi}^x_0)+ \mathbf{y}_k^\top(\boldsymbol{\psi}^y_0) \\   \mathbf{y}_k^\top (\boldsymbol{\psi}^x_0)  - \mathbf{x}_k^\top(\boldsymbol{\psi}^y_0) \end{bmatrix} \\
% &= \begin{bmatrix} \mathbf{x}_k^\top & \mathbf{y}_k^\top \end{bmatrix} \begin{bmatrix} \boldsymbol{\psi}^x_0 (\boldsymbol{\psi}^x_0)^\top + \boldsymbol{\psi}^y_0 (\boldsymbol{\psi}^y_0)^\top & \boldsymbol{\psi}^x_0 (\boldsymbol{\psi}^y_0)^\top - \boldsymbol{\psi}^y_0 (\boldsymbol{\psi}^x_0)^\top \\ \boldsymbol{\psi}^y_0 (\boldsymbol{\psi}^x_0)^\top - \boldsymbol{\psi}^x_0 (\boldsymbol{\psi}^y_0)^\top & \boldsymbol{\psi}^x_0 (\boldsymbol{\psi}^x_0)^\top + \boldsymbol{\psi}^y_0 (\boldsymbol{\psi}^y_0)^\top \end{bmatrix} \begin{bmatrix} \mathbf{x}_k \\ \mathbf{y}_k \end{bmatrix} \\
% &= 
% \begin{bmatrix} \mathbf{x}_k^\top & \mathbf{y}_k^\top \end{bmatrix}
% \left(\begin{bmatrix} \boldsymbol{\psi}^x_0 \\ \boldsymbol{\psi}^y_0 \end{bmatrix} \begin{bmatrix} (\boldsymbol{\psi}^x_0)^\top & (\boldsymbol{\psi}^y_0)^\top \end{bmatrix} + 
% \begin{bmatrix} \boldsymbol{\psi}^y_0 \\ -\boldsymbol{\psi}^x_0 \end{bmatrix} \begin{bmatrix} (\boldsymbol{\psi}^y_0)^\top & -(\boldsymbol{\psi}^x_0)^\top \end{bmatrix} \right)
% \begin{bmatrix} \mathbf{x}_k \\ \mathbf{y}_k \end{bmatrix}
% \end{align}
% and the second term becomes,
% \begin{align}
% \begin{bmatrix} \mathbf{x}_k^\top & \mathbf{y}_k^\top \end{bmatrix}
% \left(\begin{bmatrix} \cos(\lambda_k t_m) \boldsymbol{\psi}^x_m + \sin(\lambda_k t_m) \boldsymbol{\psi}^y_m \\ 
% \cos(\lambda_k t_m) \boldsymbol{\psi}^y_m - \sin(\lambda_k t_m) \boldsymbol{\psi}^x_m \end{bmatrix} 
% \begin{bmatrix} (\boldsymbol{\psi}^x_0)^\top & (\boldsymbol{\psi}^y_0)^\top \end{bmatrix} + 
% \begin{bmatrix} \cos(\lambda_k t_m) \boldsymbol{\psi}^y_m - \sin(\lambda_k t_m) \boldsymbol{\psi}^x_m  \\
% -\cos(\lambda_k t_m) \boldsymbol{\psi}^x_m - \sin(\lambda_k t_m) \boldsymbol{\psi}^y_m \end{bmatrix}  \begin{bmatrix} (\boldsymbol{\psi}^y_0)^\top & -(\boldsymbol{\psi}^x_0)^\top \end{bmatrix} \right)
% \begin{bmatrix} \mathbf{x}_k \\ \mathbf{y}_k \end{bmatrix}
% \end{align}
}

\rv{For fixed $\lambda_k$ we can calculate the analytic minimum of the loss function since we have a quadratic form. For a low rank matrix the nonzero eigenvalues of $AB^\top$ equal those of $B^\top A$ which in our case is a $4\times 4$ matrix. Defining $\mathbf{z} = [\mathbf{z}_1, \ldots, \mathbf{z}_n]$ we can write our loss in the form
\begin{equation}
L = \left \langle \left| \boldsymbol{\psi} \right|^2 \right\rangle_1 - \mathbf{z}^\top \begin{bmatrix} L_1 \\ & L_2 \\&& \ddots \\ &&& L_n \end{bmatrix} \mathbf{z}
\end{equation}
where the matrix now is of rank $4n$. We also want to impose the structures on $\mathbf{z}$ that enforce the orthogonality of the individual $\mathbf{z}_k$. We therefore seek to minimize the Lagrangian, 
\begin{align*}
L &= \left\langle |\boldsymbol{\psi}|^2 \right\rangle_1  - \sum_{k = 1}^2 \mathbf{z}_k^\top L_k \mathbf{z}_k + \lambda_1 (1 - \lVert z_1 \rvert_2^2) + \lambda_2 (1 - \lVert z_2 \rvert_2^2) - \lambda_3 z_1^\top z_2 - \lambda_4 z_1^\top \mathbb{P}_n z_2 \\
&= \lambda_1 + \lambda_2 + \left\langle |\boldsymbol{\psi}|^2 \right\rangle_1 - \mathbf{z}^\top \begin{bmatrix} L_1 + \lambda_1 \mathbb{I} & \lambda_3 \mathbb{I} + \lambda_4 \mathbb{P}_n \\ \lambda_3 \mathbb{I} - \lambda_4 \mathbb{P}_n &  L_2 + \lambda_2 \mathbb{I} \end{bmatrix} \mathbf{z}
\end{align*}}

\rv{The question remains how do we calculate the $\lambda_k$s. We consider sums of the form, 
\begin{align*}
\left\langle \boldsymbol{\psi}(0)^\top \boldsymbol{\psi}(t_m) \right\rangle_{\cos \lambda t} &= \sum_{k = 1}^n \left|Z_k^\top \boldsymbol{\psi}_0\right|^2 \left\langle \cos(\lambda_k t_m) \right\rangle_{\cos \lambda t} = \frac{1}{M} \sum_{k = 1}^n \left|Z_k^\top \boldsymbol{\psi}_0\right|^2 \sum_{m = 0}^{T - 1} \cos(\lambda_k m \Delta t) \cos(\lambda m \Delta t) \\
&= \sum_{m = 0}^{T - 1} \left(\frac{1}{M} \sum_{k = 1}^n \left|Z_k^\top \boldsymbol{\psi}_0\right|^2  \cos(\lambda_k m \Delta t) \right) \cos(\lambda m \Delta t) \\
\left\langle \boldsymbol{\psi}(0)^\top \boldsymbol{\psi}(t_m) \right\rangle_{\sin \lambda t} &= \sum_{k = 1}^n  \left|Z_k^\top \boldsymbol{\psi}_0\right|^2 \left\langle\cos(\lambda_k t_m) \right\rangle_{\sin \lambda t} = \frac{1}{M} \sum_{k = 1}^n \left|Z_k^\top \boldsymbol{\psi}_0\right|^2 \sum_{m = 0}^{T - 1} \cos(\lambda_k m \Delta t) \sin(\lambda m \Delta t) \\
&= \sum_{m = 1}^{T - 1} \left(\frac{1}{M} \sum_{k = 1}^n \left|Z_k^\top \boldsymbol{\psi}_0\right|^2  \cos(\lambda_k m \Delta t) \right) \sin(\lambda m \Delta t) 
\end{align*}
when $\boldsymbol{\psi}(t_m) = \sum_{k = 1}^n Z_k \exp(t \Lambda_k) Z_k^\top \boldsymbol{\psi}_0$ and $t_m = (m - 1)\Delta t $. From the above calculations we see that if the data is sampled at a spacing of $\Delta t$ then the averages become $2\pi/\Delta t$ periodic in $\lambda$, since $\cos((\lambda + 2\pi/\Delta t) \Delta t m)$ is indistinguishable from $\cos(\lambda \Delta t m)$, and the function is band limited. Using the Fourier series definition for a $2L$ periodic function, 
\begin{equation}
f(x) = \sum_{m = 0}^N a_m \cos(\pi m x / L) + b_m  \sin(\pi m x / L)
\end{equation}
and the Fourier series coefficients of the averages are given by
\begin{align}
a_m &= \frac{1}{M} \sum_{k = 1}^n \left|Z_k^\top \boldsymbol{\psi}_0\right|^2  \cos(\lambda_k m \Delta t), & b_m &= 0 \\
 a_m &= 0, & b_m &= \frac{1}{M} \sum_{k = 1}^n \left|Z_k^\top \boldsymbol{\psi}_0\right|^2  \cos(\lambda_k m \Delta t)
\end{align}
for $0 \le m \le T = 1$ respectively. The problem of finding $\lambda_k$ reduces to fitting a multi-tone cosine wave to the Fourier coefficients of the data -- a problem that is well studied in the signal processing literature. When the data does not perfectly fit the constrained model or there is noise present in the data then the Fourier coefficients are corrupted by noise requiring a robust fitting procedure. In general how close $a_0$ is to $1$ gives a measure of how appropriate the model is for a given data set.
}

\section{Complex analytical solution to the full model}\label{SI:analytical_solution_full}

\rv{We can perform the same analysis in the complex formulation of the problem, 
\begin{equation*}
    \dot{\boldsymbol{\psi}}_z = iH \boldsymbol{\psi}_z. 
\end{equation*}
Since $H$ is Hermitian we know that it has an eigendecompostion of the form $H = Q \Lambda Q^\dagger$ where $Q$ is a complex unitary matrix $Q^\dagger Q = Q Q^\dagger = I$ and $\Lambda$ is a real diagonal matrix. The solution of the linear ODE can therefore be written as, 
\begin{equation}
    \psi_z(t) = Q\exp(i\Lambda t) Q^\dagger \boldsymbol{\psi}_{z}^0.
\end{equation}
To fit the solution to data sampled at equally spaced time points $t_m = m \Delta t$ we minimize the loss function,
\begin{align}
    L(Q, Q^\dagger, \Lambda) &= \frac{1}{T}\sum_{m = 0}^{T - 1} \left\lVert \boldsymbol{\psi}_m - Q\exp(i\Lambda m \Delta t) Q^\dagger \boldsymbol{\psi}_z^0 \right\rVert_2^2 \\
    &= \frac{1}{T}\sum_{m = 0}^{T - 1} \left[ \boldsymbol{\psi}_m^\dagger - (\boldsymbol{\psi}_z^0)^\dagger Q\exp(-i\Lambda m \Delta t) Q^\dagger \right]\left[\boldsymbol{\psi}_m - Q\exp(i\Lambda m \Delta t) Q^\dagger \boldsymbol{\psi}_z^0\right] \\
    &= \frac{1}{T} \sum_{m = 0}^{T - 1} \left\lVert\boldsymbol{\psi}_m \right\rVert_2^2 + \left\lVert Q^\dagger \boldsymbol{\psi}_0 \right\rVert_2^2 -  (\boldsymbol{\psi}_z^0)^\dagger Q\exp(-i\Lambda m \Delta t) Q^\dagger \boldsymbol{\psi}_m - \boldsymbol{\psi}_m^\dagger Q\exp(i\Lambda m \Delta t) Q^\dagger \boldsymbol{\psi}_z^0 \\ 
    &= \frac{1}{T} \sum_{m = 0}^{T - 1} \left\lVert\boldsymbol{\psi}_m \right\rVert_2^2 + \left\lVert Q^\dagger \boldsymbol{\psi}_0 \right\rVert_2^2 -  (\boldsymbol{\psi}_z^0)^\dagger Q\exp((\Lambda_c - \Lambda_c^\dagger) m \Delta t) Q^\dagger \boldsymbol{\psi}_m - \boldsymbol{\psi}_m^\dagger Q\exp((\Lambda_c^\dagger - \Lambda_c) m \Delta t) Q^\dagger \boldsymbol{\psi}_z^0 
\end{align}
As in the real case we can rewrite this as a quadratic functional in $\mathbf{q}_k$.
}

\section{Low rank structure of the dynamical matrix}\label{SI:lowrank}

\rv{We consider the singular value decomposition of our real structured dynamical matrix,
\begin{equation*}
M = \begin{bmatrix} A & S \\ -S & A \end{bmatrix} = Z \begin{bmatrix} 0 & \Lambda \\ -\Lambda & 0 \end{bmatrix} Z^\top
\end{equation*}
Multipling both sides by $Z$ we see that, 
\begin{align*}
MZ = Z \begin{bmatrix} 0 & \Lambda \\ -\Lambda & 0 \end{bmatrix} = \begin{bmatrix} X & Y \\ Y & -X \end{bmatrix} \begin{bmatrix} 0 & \mathbb{I}_n \\ -\mathbb{I}_n & 0 \end{bmatrix} \begin{bmatrix} 0 & -\mathbb{I}_n \\ \mathbb{I}_n & 0 \end{bmatrix} \begin{bmatrix} 0 & \Lambda \\ -\Lambda & 0 \end{bmatrix} = \begin{bmatrix} -Y & X \\ X & Y \end{bmatrix} \begin{bmatrix} \Lambda & 0 \\ 0 & \Lambda \end{bmatrix}
\end{align*}
We therefore see that $Z$ provides us with $2n$ right singular vectors and the corresponding left singular vectors are given by the left matrix in the last equality. The singular values are given by $\Lambda$ and are all double degenerate.  Since we have two linearly independent singular vectors corresponding to a single singular value the SVD is not unique -- any normalized sum of the two singular vectors will also be a singular vector. This means that we can write out an exact minimum for the problem. }

\rv{For our skew-symmetric structure it only makes sense to talk about even rank approximations and we see that the best rank $2k$ approximations in the Frobenius norm sense comes from either truncating the eigendecomposition keeping the $2k$ largest magnitude eigenvalues or the truncated SVD, with both giving the same answer. }

%\section{Householder parameterization of the complex Steifel manifold (CSM)}

%\rv{We will write a complex unitary matrix $Q$ in the form $Q = H_{r - 1} H_{r - 2} \cdots H_0$
%where $H$ is the generalized complex Householder matrix paramaterized by the vector $H_k = H_k(v_k, \phi_k)$.
%$v_k$ is a vector of length $n - k$ where the first entry is purely real and is dictated by the unit norm constraint and $\phi_k$ is a real phase. 
%There are $2(n - k - 1) + 1$ degrees of freedom which gives a total number of degrees of freedom of $\sum_{k = 0}^r 2(n - k) - 1 = 2nr - r(r + 1) = 2nr - r^2$, 
%which matches the dimension of the Complex Steifel Manifold (CSM).
%$$\frac{\partial Q}{\partial v_{ki}} = H_{r - 1}\cdots H_{k + 1} \frac{\partial H_{k}}{\partial v_{ki}} H_{k - 1} \cdots H_0$$
%\begin{align*}
%H_{i, j} &= \delta_{i, j} + (e^{i\phi} - 1) v_i v_j^* \\
%\frac{\partial H}{\partial v_k} &= (e^{i\phi} - 1) e_k v^\dagger \\ 
%\frac{\partial H}{\partial v_k^*} &= (e^{i\phi} - 1) v e_k^\dagger \\ 
%\frac{\partial H}{\partial x_k} &=   (e^{i\phi} - 1) (e_k v^\dagger + v e_k^\dagger) \\
%\frac{\partial H}{\partial y_k} &= i (e^{i\phi} - 1) (e_k v^\dagger - v e_k^\dagger) \\ 
%\end{align*}
%}

